Challenges of Multilingual Program Specification and Analysis

Multilingual programs, whose implementations are made of different languages, are gaining traction especially in domains, such as web programming, that particularly benefit from the additional flexibility brought by using multiple languages. In this paper, we discuss the impact that the features commonly used in multilingual programming have on our capability of specifying and analyzing them. To this end, we first outline a few broad categories of multilingual programming, according to the mechanisms that are used for inter-language communication. Based on these categories, we describe several instances of multilingual programs, as well as the intricacies that formally reasoning about their behavior would entail. We also summarize the state of the art in multilingual program analysis, including the challenges that remain open. These contributions can help understand the lay of the land in multilingual program specification and analysis, and motivate further work in this area.

==> macros.tex <==


\usepackage{savesym}
\savesymbol{endnote}

\usepackage{booktabs}
\usepackage{listings}
\usepackage{lstautogobble}

\lstdefinestyle{displayed}{
  numbers=none, firstnumber=last, 
  breaklines=true,
  breakatwhitespace=false,         
  keepspaces=true,                 
  numbersep=2pt,
  showspaces=false,                
  showstringspaces=false,
  showtabs=false,                  
frame=tb,
  captionpos=b,                    
numberstyle=\scriptsize,
  tabsize=2,
  captionpos=b,
xleftmargin=0mm, xrightmargin=0mm, basicstyle=\ttfamily\small,
  keepspaces=true,
  columns=fixed,
  escapeinside={(*}{*)},
  mathescape=true,
  showstringspaces=false,
keywordstyle=\color{blue}\bfseries\ttfamily,
  commentstyle=\color{DarkGreen}\itshape\ttfamily,
  ndkeywordstyle=\color{purple}\bfseries,
  identifierstyle=\color{black},
  stringstyle=\color{darkgray}\ttfamily,
}

\lstdefinestyle{displayedC}{style=displayed,escapeinside={($}{$)}}
\lstdefinestyle{displayedPy}{style=displayed,mathescape=false}

\lstset{style=displayed}

\lstdefinelanguage{JavaScript}{
  morekeywords=[1]{break, continue, delete, else, for, function, if, in,
    new, return, this, typeof, var, void, while, with},
morekeywords=[2]{false, null, true, boolean, number, undefined,
    Array, Boolean, Date, Math, Number, String, Object},
morekeywords=[3]{eval, parseInt, parseFloat, escape, unescape},
  sensitive,
  morecomment=[s]{/*}{*/},
  morecomment=[l]//,
  morecomment=[s]{/**}{*/}, morestring=[b]',
  morestring=[b]"
}[keywords, comments, strings]

\newcommand{\Jc}[1]{\mbox{\lstinline[basicstyle=\ttfamily\footnotesize,language=Java]|#1|}}
\newcommand{\JSc}[1]{\mbox{\lstinline[basicstyle=\ttfamily\footnotesize,language=JavaScript]|#1|}}
\newcommand{\Sc}[1]{\mbox{\lstinline[basicstyle=\ttfamily\footnotesize,language=Scala]|#1|}}
\newcommand{\Cc}[1]{\mbox{\lstinline[basicstyle=\ttfamily\footnotesize,language=C]|#1|}}
\newcommand{\Pc}[1]{\mbox{\lstinline[basicstyle=\ttfamily\footnotesize,language=Python,mathescape=false]|#1|}}

\usepackage{enotez}

\restoresymbol{enotez}{endnote}
\setenotez{list-name={URL References}}
\setenotez{counter-format=alph}
\setenotez{mark-cs={\formatEndNoteMark}}
\setenotez{list-heading=\section*{#1}}
\newcommand{\formatEndNoteMark}[1]{\textsuperscript{\{\color{blue}{\textsf{#1}}\}}}

\DeclareDocumentCommand{\URLref}{O{} m}
{\enotezendnote{\IfNoValueF{#1}{#1\xspace}\url{#2}}}


\usepackage{graphicx}

\usepackage{dsfont}
\usepackage{latexsym}
\usepackage{csquotes}
\usepackage{tcolorbox}
\usepackage{listings}
\usepackage{float}
\usepackage{multirow}
\usepackage[scaled]{helvet}
\usepackage[noend]{algpseudocode}
\usepackage{mathrsfs}
\usepackage[linesnumbered, ruled, lined]{algorithm2e}  \usepackage{mathpartir}
\usepackage{mathtools}
\usepackage{stmaryrd}
\usepackage{textcomp} 
\usepackage{bbm}
\usepackage{verbdef}
\usepackage{xspace}
\usepackage{verbatim}
\usepackage{lipsum}
\usepackage{wrapfig}
\newcounter{tags}
\usepackage[shortlabels,inline]{enumitem}
\usepackage{pifont}
\usepackage{varwidth}
\usepackage{xpatch}
\usepackage{multirow}
\usepackage{xcolor}
\usepackage[export]{adjustbox}
\usepackage{caption}
\usepackage{subcaption}
\usepackage{setspace}
\usepackage[capitalize]{cleveref}
\usepackage{makecell}
\usepackage{dashrule}
\usepackage{comment}
\usepackage{arydshln}
\usepackage{ifsym}
\usepackage{mdframed}
\usepackage{fancyvrb}


\setlist[enumerate]{label=\emph{\roman*})}
\setlist[description]{font=\normalfont\bfseries}

\usepackage{flushend}

\usepackage{tikz}
\usetikzlibrary{calc,positioning,math,arrows,shapes,fit,intersections}
\usepackage{pgfplots}
\pgfplotsset{compat=newest}

\usepackage{xstring,xparse}

\usepackage{fontawesome}

\newcommand{\Javascript}{\emph{JavaScript}}


==> notes.tex <==
\ifdraft
\usepackage[colorinlistoftodos,textsize=scriptsize,obeyFinal,textwidth=33mm]{todonotes}

\DeclareDocumentCommand{\ReviewNote}{s o m O{white}}{\todo[color=#4,\IfBooleanTF{#1}{inline}{}]{\IfNoValueF{#2}{\textbf{#2:}\xspace}#3}
}
\else
\DeclareDocumentCommand{\ReviewNote}{s o m O{white}}{}
\fi

\newcommand{\caf}[1]{\ReviewNote[CAF]{#1}[orange!40]}


